Vilamb: Low Overhead Asynchronous Redundancy for Direct Access NVM

Vilamb provides efficient asynchronous systemredundancy for direct access (DAX) non-volatile memory (NVM) storage. Production storage deployments often use system-redundancy in form of page checksums and cross-page parity. State-of-the-art solutions for maintaining system-redundancy for DAX NVM either incur a high performance overhead or require specialized hardware. The Vilamb user-space library maintains system-redundancy with low overhead by delaying and amortizing the system-redundancy updates over multiple data writes. As a result, Vilamb provides 3--5x the throughput of the state-of-the-art software solution at high operation rates. For applications that need system-redundancy with high performance, and can tolerate some delaying of data redundancy, Vilamb provides a tunable knob between performance and quicker redundancy. Even with the delayed coverage, Vilamb increases the mean time to data loss due to firmware-induced corruptions by up to two orders of magnitude in comparison to maintaining no system-redundancy.

==> tables/design-space.tex <==
% \def\arraystretch{1.25}
\setlength{\tabcolsep}{3pt}

\begin{tabular}{r||c|c|c|c|c}
% \hline
	\makecell[r]{\textbf{DAX NVM}\\\textbf{Redundancy Solution}} & 
	\makecell[l]{\textbf{Data Update}\\\textbf{Identification}} & 
	\makecell[l]{\textbf{Redundancy}\\\textbf{Updates}} & 
	\makecell[l]{\textbf{Critical}\\\textbf{Path}\\\textbf{Interpos-}\\\textbf{itioning}} & 
	\makecell[l]{\textbf{Programming}\\\textbf{Model}}  &
	\makecell[l]{\textbf{Max. Window of}\\\textbf{Non-Redundancy}} \\ 
\hline
	\makecell[r]{Mojim~\cite{mojim-asplos}, HotPot~\cite{hotpot-socc}} & 
	\makecell[l]{Application\\Instrumentation} & 
	\makecell[l]{Transaction\\Boundaries} & 
	\makecell[l]{Yes} & 
	\makecell[l]{Restrictive}  &
	\makecell[l]{None} \\
 \hline
	\makecell[r]{Mojim, HotPot augmented \\ with Lazy Redundancy} & 
	\makecell[l]{Application\\Instrumentation} & 
	\makecell[l]{Lazily} & 
	\makecell[l]{Yes} & 
	\makecell[l]{Restrictive}  &
	\makecell[l]{Configurable} \\ 
 \hline 
	\makecell[r]{\system w/ Volatile\\Dirty Bits (\cref{sec:wp})} & 
	\makecell[l]{Write Protection} & 
	\makecell[l]{Lazily} & 
	\makecell[l]{Yes} & 
	\makecell[l]{Non-restrictive}  &
	\makecell[l]{Configurable} \\ 
 \hline 
	\makecell[r]{\system} & 
	\makecell[l]{Dirty Bits} & 
	\makecell[l]{Lazily} & 
	\makecell[l]{No} & 
	\makecell[l]{Non-restrictive}  &
	\makecell[l]{Configurable} \\ 
% \hline 
\end{tabular}


==> tables/reliability-notation.tex <==
% \def\arraystretch{1.25}
{\footnotesize
\setlength{\tabcolsep}{3pt}

\begin{tabular}{r|l}
	\makecell[r]{\textbf{Notation}} & 
	\makecell[l]{\textbf{Description}}\\  
\Xhline{2\arrayrulewidth}
	\makecell[r]{$\mttfpage$} & 
	\makecell[l]{Mean Time To Page Failue (Corruption)}\\ 
\hline
	\makecell[r]{$\mttfdimm$} & 
	\makecell[l]{Mean Time To (DIMM) Failure}\\ 
\hline
	\makecell[r]{$\numpages$} & 
	\makecell[l]{Total Number of Pages}\\
\hline
	\makecell[r]{$\numdimms$} & 
	\makecell[l]{Number of DIMMs / Stripe Width}\\
\hline
	\makecell[r]{$\dataperdimm$} & 
	\makecell[l]{Data Per DIMM}\\
\hline
	\makecell[r]{$\fraction$} & 
	\makecell[l]{Average Uncovered Data Fraction}\\ %\\with redundancy update period $p$}\\
%	
%\hline
%	\makecell[l]{\mttfdimm} & 
%	\makecell[l]{DIMM Mean Time To Failure}\\
%\hline
%	\makecell[l]{\numdimms} & 
%	\makecell[l]{Total Number of DIMMs (N data + 1 parity DIMM)}\\
%\hline
%	\makecell[l]{\pagesperdimm} & 
%	\makecell[l]{Number of Pages per DIMM}\\
%\hline
%	\makecell[l]{\pagesize} & 
%	\makecell[l]{Page Size}\\
%\hline
%	\makecell[l]{\mttrpage} & 
%	\makecell[l]{DIMM Mean Time To Recovery}\\
\end{tabular}
}

